Non-perturbative renormalisation of left-left four-fermion operators with Neuberger fermions

We outline a general strategy for the non-perturbative renormalisation of composite operators in discretisations based on Neuberger fermions, via a matching to results obtained with Wilson-type fermions. As an application, we consider the renormalisation of the four-quark operators entering the Delta S=1 and Delta S=2 effective Hamiltonians. Our results are an essential ingredient for the determination of the low-energy constants governing non-leptonic kaon decays.

==> tables.tex <==
%\begin{table}[!t]
%\begin{center}
%\begin{tabular}{ccccccc}
%\Hline \\[-10pt]
%$\beta$ & $(L/a)^3 \times T/a$ & $\frac{a}{2r_0}$ & $\frac{L}{2r_0}$  & $\kappa_s$ & 
%$(\kappa_d,a\mu)$ & $N_{\rm conf}$\\
%&&&&&& \\[-10pt]
%\hline \\[-10pt]
%6.0 & $16^3 \times 48$ & 0.0931 & 1.49 & 0.1335 & (0.135169,0.03816) & 402 \\
%& & & & 0.1338 & (0.135178,0.03152) & 398 \\
%& & & & 0.1340 & (0.135183,0.02708) & 402 \\
%& & & & 0.1342 & (0.135187,0.02261) & 400 \\ \\[-10pt]
%\hline\\[-10pt]
%6.1 & $24^3 \times 56$ & 0.0789 & 1.89 & 0.1343 & (0.1354817,0.0279110) & 100 
%\\
%& & & & 0.1345 & (0.1354860,0.0233010) & 99 \\
%& & & & 0.1347 & (0.1354896,0.0186678) & 122 \\ \\[-10pt]
%\hline\\[-10pt]
%6.2 & $24^3 \times 64$ & 0.0677 & 1.63 & 0.1346 & (0.1357800,0.0283240) & 200 
%\\
%& & & & 0.1347 & (0.1357825,0.0259850) & 201 \\
%& & & & 0.1349 & (0.1357866,0.0212897) & 214 \\ \\[-10pt]
%\hline\\[-10pt]
%6.3 & $24^3 \times 72$ & 0.0587 & 1.41 & 0.1348 & (0.1358118,0.0246230) & 200 
%\\
%    &                  &       &      & 0.1349 & (0.1358139,0.0222430) & 205 
%\\
%    &                  &       &      & 0.1350 & (0.1358157,0.0198558) & 175 
%\\
%    &                  &       &      & 0.1351 & (0.1358174,0.0174640) & 201 
%\\ \\[-10pt]
%\Hline\\[10pt]
%\end{tabular}
%\begin{tabular}{cccccc}
%\Hline \\[-10pt] 
%$\beta$ & $(L/a)^3 \times T/a$ & $\frac{a}{2r_0}$ & $\frac{L}{2r_0}$ & $(\kappa,a\mu)$ & $N_{\rm conf}$\\ 
%\\[-10pt]
%\hline \\[-10pt]
%6.00 & $24^3 \times 48$ & 0.0931 & 2.24 & (0.134739,0.010412) & 200 \\
%& & & & (0.134795,0.009142) & \\
%& & & & (0.134828,0.008397) & \\ \\[-10pt]
%\hline \\[-10pt]
%6.10 & $24^3 \times 60$ & 0.0789 & 1.89 & (0.135152,0.00810) & 200 \\
%& & & & (0.135190,0.00720) & \\
%& & & & (0.135235,0.00615) & \\ \\[-10pt]
%\hline \\[-10pt]
%6.20 & $32^3 \times 72$ & 0.0677 & 2.17 & (0.135477,0.007595) & 73 \\
%& & & & (0.135539,0.006125) & \\ \\[-10pt]
%\hline \\[-10pt]
%6.30 & $32^3 \times 72$ & 0.0587 & 1.88 & (0.135509,0.0076) & 76 \\
%& & & & (0.135546,0.0067) & \\
%& & & & (0.135584,0.0058) & \\ \\[-10pt]
%\hline \\[-10pt]
%6.45 & $32^3 \times 86$ & 0.0481 & 1.54 & (0.135105,0.01459) & 105 \\
%& & & & (0.135218,0.01185) & \\
%& & & & (0.135293,0.01002) & \\ \\[-10pt]
%\Hline
%\end{tabular}
%\end{center}
%\caption{The parameters of the runs at $(\pi/2)$ (upper table) and $(\pi/4)$ (lower table).}
%\label{tab:run_pars}
%\end{table}

%
%\newpage


%%%% FINAL RESULTS OF CARLOS' ANALYSIS AS OF 14/07/06 FOLLOW

\begin{table}[!t]
\begin{center}\scriptsize
\begin{tabular}{ccllll}
\Hline \\[-6pt] 
$\beta$ & $\big [ \dfrac{x_0^{\rm min}}{2r_0}, \dfrac{x_0^{\rm max}}{2r_0} \big ]$ &
$\,r_0 m_{\rm PS}$ & $~~~~~~~~~\cR_+$ & $~~~~~~~~~\cR_-$  & $\cR_+/\cR_-$ \\
&&&&& \\[-6pt]
\hline \hline \\[-6pt]
6.0 & $[1.30,3.17]$ & 2.092(6)  & 1.569(12)(11)(17) & 2.632(32)(19)(37) & 0.596(7) \\ \\[-6pt]
                  & & 1.907(7)  & 1.519(18)(11)(21) & 2.732(43)(19)(47) & 0.556(10) \\ \\[-6pt]
                  & & 1.780(6)  & 1.498(18)(11)(21) & 2.809(45)(20)(49) & 0.533(9) \\ \\[-6pt]
                  & & 1.635(6)  & 1.445(17)(10)(20) & 2.852(46)(20)(50) & 0.507(9) \\ \\[-6pt]
\hline \\[-6pt]
                  & & 1.2544    & 1.376(25)(31)     & 3.009(66)(73)     & 0.449(13) \\ \\[-6pt]
\hline \hline \\[-6pt]
6.1 & $[1.34,3.08]$ & 2.039(6)  & 1.433(11)(10)(15) & 2.450(27)(17)(32) & 0.585(7) \\ \\[-6pt]
                  & & 1.874(7)  & 1.380(13)(10)(16) & 2.627(32)(19)(37) & 0.525(7) \\ \\[-6pt]
                  & & 1.715(6)  & 1.332(12)(9)(16)  & 2.697(40)(19)(44) & 0.494(9) \\ \\[-6pt]
\hline \\[-6pt]
                  & & 1.2544    & 1.219(28)(37)     & 2.917(83)(94)     & 0.382(19) \\ \\[-6pt]
\hline \hline \\[-6pt]
6.2 & $[1.29,3.05]$ & 2.079(6)  & 1.364(10)(10)(14) & 2.414(28)(17)(32) & 0.565(7) \\ \\[-6pt]
                  & & 1.980(7)  & 1.323(12)(9)(15)  & 2.449(30)(17)(34) & 0.540(8) \\ \\[-6pt]
                  & & 1.795(7)  & 1.300(11)(9)(15)  & 2.623(39)(19)(43) & 0.496(8) \\ \\[-6pt]
\hline \\[-6pt]
                  & & 1.2544    & 1.203(31)(43)     & 2.92(10)(12)      & 0.393(23) \\ \\[-6pt]
\hline \hline \\[-6pt]
6.3 & $[1.23,3.00]$ & 2.050(9)  & 1.320(16)(9)(18)  & 2.352(39)(17)(43)  & 0.561(11) \\ \\[-6pt]
                  & & 1.962(8)  & 1.328(20)(9)(22)  & 2.506(45)(18)(49)  & 0.530(10) \\ \\[-6pt]
                  & & 1.839(10) & 1.278(22)(9)(24)  & 2.489(56)(18)(59)  & 0.514(12) \\ \\[-6pt]
                  & & 1.722(9)  & 1.224(20)(9)(21)  & 2.661(58)(19)(61)  & 0.460(11) \\ \\[-6pt]
\hline \\[-6pt]
                  & & 1.2544    & 1.127(43)(46)    & 2.95(12)(12)       & 0.361(25) \\ \\[-6pt]
\Hline \\[-6pt]
\end{tabular}
\end{center}
\caption{
Results for the pseudoscalar mass and the ratios $\cR_\pm$ from the $(\pi/2)$ tmQCD regularisation. The error in $r_0 m_{\rm PS}$ is statistical. The three errors
of the $R_B$ ratio are, in order of appearance: (i) due to the statistical
fluctuations of the correlations; (ii) due to the errors of 
$Z_{\rm A,V}$; (iii) the total error from the two previous ones. The results of the
extrapolations to the physical kaon mass values are shown at the bottom of
each $\beta$-dataset: the first error is that arising from
type-(i) errors of the fitted values, while the second is from type-(iii) errors.
}
\vskip 0.2cm
\label{tab:respi2}
\end{table}


\newpage


\begin{table}[!t]
\begin{center}\scriptsize
\begin{tabular}{cccccc}
\Hline \\[-6pt] 
$\beta$ & $\big [ \dfrac{x_0^{\rm min}}{2r_0}, \dfrac{x_0^{\rm max}}{2r_0} 
\big ]$ &
$r_0 m_{\rm PS}$ & $\cR_+$ & $\cR_-$  & $\cR_+/\cR_-$ \\ \\[-6pt]
\hline \\[-6pt]
6.0 & $[1.30,3.17]$ & 1.323(4)  & 1.423(10)(10)(14) & 3.202(40)(23)(46)  & 0.444(6) \\ \\[-6pt]
    & $[1.30,3.17]$ & 1.250(4)  & 1.397(11)(10)(15) & 3.306(47)(23)(53)  & 0.423(6) \\ \\[-6pt]
    & $[1.30,3.17]$ & 1.204(5)  & 1.381(12)(10)(15) & 3.379(54)(24)(59)  & 0.409(7) \\ \\[-6pt]
\hline \\[-6pt]
                  & & 1.2544    & 1.398(11)(15)     & 3.304(46)(51)      & 0.424(6) \\ \\[-6pt]
\hline\hline \\[-6pt]
6.1 & $[1.18,3.55]$ & 1.233(6)  & 1.239(14)(9)(16)  & 3.199(67)(23)(71)  & 0.387(9) \\ \\[-6pt]
    & $[1.18,3.55]$ & 1.168(6)  & 1.218(15)(9)(17)  & 3.296(77)(23)(80)  & 0.370(10) \\ \\[-6pt]
    & $[1.26,3.47]$ & 1.086(6)  & 1.190(17)(8)(19)  & 3.429(91)(24)(94)  & 0.347(10) \\ \\[-6pt]
\hline \\[-6pt]
                  & & 1.2544    & 1.247(12)(15)     & 3.160(62)(66)      & 0.394(8) \\ \\[-6pt]
\hline\hline \\[-6pt]
6.2 & $[1.35,3.52]$ & 1.300(6)  & 1.176(14)(8)(17)  & 2.999(58)(21)(61)  & 0.392(9) \\ \\[-6pt]
    & $[1.35,3.52]$ & 1.183(6)  & 1.136(17)(8)(18)  & 3.127(72)(22)(75)  & 0.364(10) \\ \\[-6pt]
\hline \\[-6pt]
                  & & 1.2544    & 1.160(14)(16)     & 3.050(62)(66)      & 0.381(9) \\ \\[-6pt]
\hline\hline \\[-6pt]
6.3 & $[1.29,2.94]$ & 1.336(10) & 1.135(18)(8)(19)  & 2.964(64)(21)(68)  & 0.383(11) \\ \\[-6pt]
    & $[1.35,2.88]$ & 1.257(10) & 1.110(19)(8)(20)  & 3.056(73)(22)(76)  & 0.363(11) \\ \\[-6pt]
    & $[1.47,2.76]$ & 1.173(10) & 1.081(20)(8)(21)  & 3.164(85)(22)(88)  & 0.342(11) \\ \\[-6pt]
\hline \\[-6pt]
                  & & 1.2544    & 1.108(18)(20)     & 3.065(72)(75)      & 0.362(10) \\ \\[-6pt]
\hline\hline \\[-6pt]
6.45& $[1.30,2.84]$ & 2.053(9)  & 1.250(15)(9)(17)  & 2.262(41)(16)(44)  & 0.553(10) \\ \\[-6pt]
    & $[1.25,2.88]$ & 1.848(10) & 1.206(17)(9)(19)  & 2.384(53)(17)(56)  & 0.506(12) \\ \\[-6pt]
    & $[1.30,2.84]$ & 1.702(10) & 1.171(18)(8)(20)  & 2.484(66)(18)(68)  & 0.472(13) \\ \\[-6pt]
\hline \\[-6pt]
                  & & 1.2544    & 1.094(23)(25)     & 2.700(93)(95)      & 0.391(17) \\ \\[-6pt]
\Hline
\end{tabular}
\end{center}
\caption{
Results for the pseudoscalar mass and the ratios $\cR_\pm$ from the $(\pi/4)$ tmQCD regularisation. The error in $r_0 m_{\rm PS}$ is statistical. The three errors
of the $R_B$ ratio are, in order of appearance: (i) due to the statistical
fluctuations of the correlations; (ii) due to the errors of 
$Z_{\rm A,V}$; (iii) the total error from the two previous ones. The results of the
extrapolations to the physical kaon mass values are shown at the bottom of
each $\beta$-dataset: the first error is that arising from
type-(i) errors of the fitted values, while the second is from type-(iii) errors.
}
\label{tab:respi4}
\end{table}





 
